FGGM: Formal Grey-box Gradient Method for Attacking DRL-based MU-MIMO Scheduler

In 5G mobile communication systems, MU-MIMO has been applied to enhance spectral efficiency and support high data rates. To maximize spectral efficiency while providing fairness among users, the base station (BS) needs to selects a subset of users for data transmission. Given that this problem is NP-hard, DRL-based methods have been proposed to infer the near-optimal solutions in real-time, yet this approach has an intrinsic security problem. This paper investigates how a group of adversarial users can exploit unsanitized raw CSIs to launch a throughput degradation attack. Most existing studies only focused on systems in which adversarial users can obtain the exact values of victims' CSIs, but this is impractical in the case of uplink transmission in LTE/5G mobile systems. We note that the DRL policy contains an observation normalizer which has the mean and variance of the observation to improve training convergence. Adversarial users can then estimate the upper and lower bounds of the local observations including the CSIs of victims based solely on that observation normalizer. We develop an attacking scheme FGGM by leveraging polytope abstract domains, a technique used to bound the outputs of a neural network given the input ranges. Our goal is to find one set of intentionally manipulated CSIs which can achieve the attacking goals for the whole range of local observations of victims. Experimental results demonstrate that FGGM can determine a set of adversarial CSI vector controlled by adversarial users, then reuse those CSIs throughout the simulation to reduce the network throughput of a victim up to 70\% without knowing the exact value of victims' local observations. This study serves as a case study and can be applied to many other DRL-based problems, such as a knapsack-oriented resource allocation problems.

==> resource/p2.tex <==
\subsubsection{Selfish user problem}
    The main goal of selfish user in this problem is trying to maximize the chance that they are selected, while minimize the chance other users is selected.
    Given the knowledge about the proto action space, the cluster head can pre-calculate what is the region in the proto action that contain the most number of adversaries, while minimize number of normal users.
    In particular, we compute the centroid that contain the most amount of adversaries by
    \begin{equation}
        \tilde{u} = \sum_{i=1}^{|\mathcal{A}|} \frac{\text{number of adversaries in set i}}{\text{number of users in set i}} u_i
    \end{equation}
    Then, the we can formulate the problem as
    \begin{problem}{Selfish users \gls{qos} (P2)}
        \begin{equation}
            \underset{\tilde{o}^t_{\text{adv}}}{\text{minimize}}
            \quad  \frac{1}{2} ( \frac{1}{2}(\tilde{u}^t_\le + \tilde{u}^t_\ge) - \tilde{u} )^2
        \end{equation}
        subject to
        \begin{equation}
            \tilde{u}^t_\ge, \tilde{u}^t_\le = \text{DP}(\pi(.|o_t; \theta),
                                                         <\tilde{o}^t_{\text{adv}}, \underbar{o}^t_{\text{vic}}>,
                                                         <\tilde{o}^t_{\text{adv}}, \bar{o}^t_{\text{vic}}>)
        \end{equation}
        \begin{equation}
            \tilde{o}^t_{\text{adv}} \ge \bar{o}^t_{\text{vic}}
        \end{equation}
        \begin{equation}
            \tilde{o}^t_{\text{adv}} \le \underbar{o}^t_{\text{vic}}
        \end{equation}
    \end{problem}
    This problem is converted minimizing the mean square error towards the centroid that contain the most amount of adversaries.

        Attacker is only one user, with it's accomplice to support itself.
        Goal is maximize the throughput of one user only.

\subsection{Suggested Countermeasures}
    \hl{TODO later}.
    First counter-measurement come to my mind is adversarial training.
    Training with the adversarial input like our is stronger than just training with \gls{fgsm} \cite{huang2017adversarial, goodfellow2014explaining, madry2017towards, dong2018boosting} or \gls{pgd}.
    Disable gradient make attacking slower, so recommend traditional heuristic or using state that not differentiable like SMART \cite{an2023deep} without vanilla version.
    Training encoder like \cite{sahay2023defending} risk having event the autoencoder being attacked.
    However, defending is outside of our scope.


==> section/util/ack.tex <==
\section*{Acknowledgement}
\tvn{Remove this entire section.  Should not have it at submission time. Can easily identify authors with grant numbers.}
This work is partially supported by XXX with grant number XXXX.



==> section/util/glossary.tex <==
% \newacronym{bs}{BS}{base station} % bo 
% \newacronym{ap}{AP}{access point} % bo
% \newacronym{zf}{ZF}{zero forcing} % bo
% \newacronym{rb}{RB}{resource block} % bo
% \newacronym{ue}{UE}{user equipment} % bo
\newacronym{dos}{DoS}{denial of service}
\newacronym{qos}{QoS}{quality of service}
% \newacronym{jfi}{JFI}{Jain fairness index} % bo
\newacronym{optmr}{\texttt{OptMR}}{optimal max rate}
\newacronym{tdd}{TDD}{time division duplexing}
\newacronym{csi}{CSI}{channel state information}
% \newacronym{csirs}{CSI-RS}{CSI reference signal} % bo
% \newacronym{awgn}{AWGN}{additive white Gaussian noise} % bo
\newacronym{mimo}{MIMO}{multiple-input multiple-output}
\newacronym{optpf}{\texttt{OptPF}}{optimal proportional fairness}
\newacronym{optpfug}{\texttt{OptPFUG}}{optimal proportional fairness with user grouping}
\newacronym{sinr}{SINR}{signal to interference-plus-noise ratio}
\newacronym{ofdm}{OFDM}{orthogonal frequency division multiplexing}
\newacronym{mumimo}{MU-MIMO}{multiple-user multiple-input multiple-output}
\newacronym{quadriga}{QuaDRiGa}{Quasi Deterministic Radio Channel Generator}

\newacronym{sac}{\texttt{SAC}}{soft actor critic}
\newacronym{knn}{KNN}{$k$ nearest neighbor}
\newacronym{dnn}{DNN}{deep neural network}
\newacronym{mdp}{MDP}{Markov decision process}
\newacronym{relu}{ReLU}{rectified linear unit}
\newacronym{tsp}{TSP}{travelling salesman problem}
\newacronym{drl}{DRL}{deep reinforcement learning}
\newacronym{ddpg}{DDPG}{deep deterministic policy gradient}
\newacronym{madrl}{MADRL}{multi-agent deep reinforcement learning}

\newacronym{pgd}{PGD}{projected gradient descent}
\newacronym{fgsm}{FGSM}{fast gradient sign method}
\newacronym{uap}{UAP}{universal adversarial perturbation}
\newacronym{mifgsm}{MI-FGSM}{momentum iterative fast gradient sign method}

\newacronym{ilp}{ILP}{integer linear programming}
\newacronym{smt}{SMT}{satisfiability modulo theory}
\newacronym{dpll}{DPLL}{Davis-Putnam-Logemann-Loveland}
\newacronym{milp}{MILP}{mixed integer linear programming}

\newacronym{spgd}{\texttt{SPGD}}{sampling-based projected gradient descent}
\newacronym{fggm}{\texttt{FGGM}}{\underline{F}ormal \underline{G}reybox \underline{G}radient \underline{M}ethod}

